Stellar populations in local AGNs: evidence for enhanced star formation in the inner 100pc

In modern models and simulations of galactic evolution, the star formation in massive galaxies is regulated by an ad hoc active galactic nuclei (AGN) feedback process. However, the physics and the extension of such effects on the star formation history of galaxies is matter of vivid debate. In order to shed some light in the AGN effects over the star formation, we analyzed the inner 500$\times$500pc of a sample of 14 Seyfert galaxies using GMOS and MUSE integral field spectroscopy. We fitted the continuum spectra in order to derive stellar age, metallicity, velocity and velocity dispersion maps in each source. After stacking our sample and averaging their properties, we found that the contribution of young SP, as well as that of AGN featureless continuum both peak at the nucleus. The fraction of intermediate-age SPs is smaller in the nucleus if compared to outer regions, and the contribution of old SPs vary very little within our field of view (FoV). We also found no variation of velocity dispersion or metallicity within our FoV. Lastly, we detected an increase in the dust reddening towards the center of the galaxies. These results lead us to conclude that AGN phenomenon is usually related to a recent star formation episode in the circumnuclear region.

==> Stellar populations in local AGNs_ evidence for enhanced star formation in the inner 100pc/figures.tex <==
\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{mrk1066.pdf}
    \caption{Stellar population results for the SB0 Seyfert\,2 galaxy Mrk\,1066. In the first row, we show the continuum emission in the first left panel. Over this panel the white arrow represents north, whereas east is represented by the small line. In the second panel, we show the percentage contribution from a Featureless continuum, with contours drawn at 10, 20, 40 and 80\%. In the third panel, we show an RGB map composed by the the detected stellar population, where blue represents the young SPs, green the intermediate-age SPs and red the old SPs. The logarithm of the mean age in years is presented in the fourth panel, and the V band dust reddening in magnitudes is presented in the fifth panel. In the second row, we show the observed and modeled stellar velocity (in units of km\,s$^{-1}$) in the first and second panels, respectively, with the residual between the observed and modeled velocities presented in the third panel. Over the modeled V panel, the gray dashed line represents the zero velocity line. In the fourth panel, we show the stellar $\sigma$ in km\,s$^{-1}$, and the metallicity is presented in the last panel in units of solar metallicity.}
    \label{fig:m1066}
\end{figure*}



\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{mrk607.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for Sa Seyfert\,2 galaxy Mrk\,607.}
    \label{fig:m607}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc1052.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for E4 LINER/Seyfert galaxy NGC\,1052.}
    \label{fig:n1052}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc1068.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for SAb Seyefrt\,2 galaxy NGC\,1068.}
    \label{fig:n1068}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc1194.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for SA Seyfert\,1 galaxy NGC\,1194.}
    \label{fig:n1194}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc2110.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for S0 Seyfert\,2 galaxy NGC\,2110.}
    \label{fig:n2110}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc2992.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for Sa Seyfert\,2 galaxy NGC\,2992.}
    \label{fig:n2992}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc3081.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for S0 Seyfert\,2 galaxy NGC\,3081.}
    \label{fig:n3081}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc3393.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for Sa Seyfert\,2 galaxy NGC\,3393.}
    \label{fig:n3393}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc3516.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for SB0 Seyfert\,1.5 galaxy NGC\,3516.}
    \label{fig:n3516}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc3786.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for SA Seyfert\,1.8 galaxy NGC\,3786.}
    \label{fig:n3786}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc4939.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for Sbc Seyfert\,1 galaxy NGC\,4939.}
    \label{fig:n4939}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc5728.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for SBb Seyfert\,2 galaxy NGC\,5728.}
    \label{fig:n5728}
\end{figure*}

\begin{figure*}
    %\centering
    \includegraphics[width=\textwidth]{ngc5899.pdf}
    \caption{Same as Fig~\ref{fig:m1066}, but for SAB Seyfert\,2 galaxy NGC\,5899.}
    \label{fig:n5899}
\end{figure*}

